The Complexity of Network Satisfaction Problems for Symmetric Relation Algebras with a Flexible Atom

Robin Hirsch posed in 1996 the 'Really Big Complexity Problem': classify the computational complexity of the network satisfaction problem for all finite relation algebras A. We provide a complete classification for the case that A is symmetric and has a flexible atom; in this case, the problem is NP-complete or in P. The classification task can be reduced to the case where A is integral. If a finite integral relation algebra has a flexible atom, then it has a normal representation B. We can then study the computational complexity of the network satisfaction problem of A using the universal-algebraic approach, via an analysis of the polymorphisms of B. We also use a Ramsey-type result of Ne\v{s}et\v{r}il and R\"odl and a complexity dichotomy result of Bulatov for conservative finite-domain constraint satisfaction problems.

==> BinaryInjections6.tex <==
%!TEX root = ClassificationFlexAtomsAlgebras.tex


\section{Binary Injections}\label{section:binary injection}
We give in this section a proof of the following proposition.

\begin{proposition}%\label{binaryinjectionNPhard}
	Let $\mathfrak{B}$ be a normal representation of a finite, symmetric, integral  $\mathbf{A}\in \rra$ with a flexible atom $s$. If $\mathfrak{B}$ does not have a binary injective polymorphism, then $\HSPf(\{\Pol(\mathfrak{B }) \}  )$ contains a 2-element algebra where all operations are projections. Therefore, $\csp(\mathfrak{B})$ is NP-complete.
\end{proposition}


Note that an injective polymorphism of $\mathfrak{B}$ is $\{a,\id\}$-canonical, and even $\{a,\id\}$-symmetric for all atoms $a\in A_0$ since polymorphisms of a normal representation are edge-conservative.

We first apply the independence lemma on the pair $\{s,\id\}$ of atoms where $s$ is the flexible atom and analyze the situation when no $\{s,\id\}$-symmetric polymorphism exists. The outcome is that this is sufficient for the NP-hardness.
 We will see in Lemma \ref{lemma:not(2) implies no symm} that in order to prove Proposition \ref{binaryinjectionNPhard} this is enough, since the absence of a binary injective polymorphism implies the absence of an  $\{s,\id\}$-symmetric polymorphism.
%In Section \ref{subsection:a id canon} we apply the independence lemma on a pair $\{a,\id\}$ of atoms and analyze the situation when no $\{a,\id\}$-symmetric polymorphism exists.
% In Section \ref{subsection:special independece} we prove a slightly different independence lemma. This lemma will not only take two atomic relation into account and is in some sense the classical independence lemma with an injective operation as functional part.





%IST IM APPENDIX


\begin{lemma}\label{lem: make things unequal}
	Let $\mathfrak{B}$ be a normal representation of a finite, integral, symmetric $\mathbf{A}\in\rra$ with a flexible atom $s$. 
	Let $\psi$ be the formula $$\psi(x_1,x_2,y_1,y_2):=\overline{\id}(x_1,y_1)\wedge \overline{\id}(x_1,y_2)\wedge \overline{\id}(x_2,y_1)\wedge \overline{\id}(x_2,y_2).$$
	
	 
Let  $\varphi$ be a primitive positive formula such that 
$\varphi \wedge s(x_1,x_2)   \wedge  \id(y_1,y_2)$ and $\varphi \wedge \id(x_1,x_2)  \wedge s(y_1,y_2)$
are satisfiable over $\mathfrak{B}$, but the formula $\varphi \wedge s(x_1,x_2)   \wedge  s(y_1,y_2)$ is not satisfiable over $\mathfrak{B}$.
Then there exists a primitive positive formula $\varphi'$ such that
 
 \begin{align*}
 &\varphi'\wedge\psi(x_1,x_2,x_3,x_4) \wedge s(x_1,x_2)   \wedge  \id(y_1,y_2)\\
 \text{and } &\varphi' \wedge\psi(x_1,x_2,x_3,x_4)\wedge \id(x_1,x_2)  \wedge s(y_1,y_2)
 \end{align*}
 are satisfiable over $\mathfrak{B}$  and the formula $\varphi \wedge s(x_1,x_2)   \wedge  s(y_1,y_2)$ is not satisfiable over $\mathfrak{B}$ (we denote this property with $\bigstar$).
\end{lemma}



\begin{proof}
	
	Let $R_{\id}$ be the ternary relation defined by the formula
	$$\sigma(x_1,x_2,x_3):= (s\cup\id)(x_1,x_2) \wedge (s\cup\id)(x_2,x_3)  \wedge s(x_1,x_2) .$$
	
	For this formula it holds that $\sigma \wedge s(x_1,x_2)   \wedge  \id(x_2,x_3)$ and $\sigma \wedge \id(x_1,x_2)  \wedge s(x_2,x_3)$
	are satisfiable, but the formula $\sigma\wedge \id(x_1,x_2)   \wedge  \id(x_2,x_3)$ is not satisfiable.
	
	
	
	Assuming the statement of the lemma does not hold for $\varphi$ we consider the following cases. Without loss of generality we may assume that $\varphi \wedge s(x_1,x_2)   \wedge  \id(y_1,y_2) \wedge \id(x_2,y_1)$ holds. Otherwise, we may change the roles of some variables.
	
	
	
	\begin{enumerate}
		\item $\varphi \wedge \id(x_1,x_2)   \wedge  s(y_1,y_2) \wedge \id(x_2,y_1)$ is satisfiable.
		\item $\varphi \wedge \id(x_1,x_2)   \wedge  s(y_1,y_2) \wedge c(x_2,y_1) \wedge b(x_1,y_4)$ is satisfiable for atoms $c,b\in A_0\setminus\{s\}$.
		\item $\varphi \wedge \id(x_1,x_2)   \wedge  s(y_1,y_2) \wedge \id(x_1,y_2) $ is satisfiable.
	\end{enumerate}
We prove the statement for these cases.
\medskip

\underline{Case 1:} Let $R_s$ be the ternary relation defined by $\sigma'(x_1,x_2,y_2):= \varphi(x_1,x_2,x_2,y_2)$. 
Then $\sigma'\wedge s(x_1,x_2)   \wedge  \id(x_2,y_2)$ and $\sigma'\wedge \id(x_1,x_2)  \wedge s(x_2,y_2)$
are satisfiable, but the formula $\psi \wedge s(x_1,x_2)   \wedge  s(x_2,y_2)$ is not satisfiable (we denote this with property $\spadesuit$).
Consider the following formula:
\begin{align*}\label{defi varphi'}
\varphi'(x_1,x_2,y_1,y_2):= \exists z: (R_s(x_1,x_2,yz\wedge R_{\id}(x_2,z,y_1) \wedge R_{s}(z,y_1,y_2)).
\end{align*}
We show that $\varphi$ has property $\bigstar$. Consider the following substructure of $\mathfrak{B }$ on elements $a^1,a^2$ and $a^2$ such that the atomic relations that hold on this structure are $$s(a^1,a^2) , ~s(a^2,a^3), \text{~and~}s(a^1,a^3).$$
Then $\varphi'(a^1,a^2,a^3,a^3)$ holds in $\mathfrak{B }$ if we choose $a^2$ for the variable $z$. Therefore we get:



$$\varphi'(a^1,a^2,a^3,a^3)\wedge\psi(a^1,a^2,a^3,a^3) \wedge s(a^1,a^2)   \wedge  \id(a^3,a^3).$$ 
This shows the first satisfiability part of property $\bigstar$. The other satisfiability part holds also since we can choose the tuple $(a^1,a^1,a^2,a^3)$ by an analogous argument. 
The non-satisfiability part of $\bigstar$ follows by the definition of $\varphi'$.
Assuming $s(x_1,x_2)$ and $s(y_1,y_2)$ hold we get by the properties of $R_s$ that $\id(x_2,z)$ and $\id(z,y_1)$ hold. This contradicts the properties of $R_{\id}$.
Therefore we finished Case~1.



\medskip
\underline{Case 2:}
Consider the formula
$$\varphi'(x_1,x_2,y_1,y_2):= \exists z_1,z_2,z_3: \varphi(x_1,x_2,z_1,z_2) \wedge R_{\id}(z_1,z_2,z_3) \wedge \varphi(z_2,z_3,y_1,y_2).$$
We show that $\varphi'$ has property $\bigstar$. Let $a^1, \ldots, a^4\in B$ such that the following relations hold:$$ s(a^1,a^2), s(a^2,a^3), c(a^3,a^4) , s(a^1,a^4), s(a^1,a^3)\text{~and~} b(a^2,a^4) . $$
Such a substructure clearly exists since $s$ is a flexible atom.
We claim that the tuple $(a^1,a^2,a^4,a^4)$  is a witness that $\varphi'$ satisfies the first satisfiability part of property $\bigstar$. To see this, choose for the existentially quantified variables $z_1,z_2$ and $z_3$ the elements $a^2, a^2$ and $a_3$. It is easy to check that $(a^1,a^2,a^2,a^2)$ and $(a^2,a^3,a^4,a^4)$ satisfy $\varphi$ and that $(a^2,a^2,a^3) \in R_{\id}$ holds.
The second satisfiability statement in property $\bigstar$ follows by an analogous argument.
The non-satisfiability part is clear by the definition and the same argument as for Case~1.

\medskip
\underline{Case 3:}
Consider the ternary relation $R_s$ defined by $$\sigma(x_1,x_2,x_3):=\exists z: ( \varphi(x_1,x_2,x_3,z) \wedge \id(x_2,y_2)\wedge (\id\cup s)(y_1,y_2)).$$ This relation and its defining formula have property $\spadesuit$. Therefore the proof is the same as in Case~1. \qed\end{proof}



\begin{lemma}\label{lemma: no a id symm implies a id canonical}
	Let $\mathfrak{B}$ be a normal representation of a finite, integral, symmetric  $\mathbf{A}\in \rra$ with a flexible atom $s$. If there exists no $\{s,\id\}$-symmetric polymorphism, then all polymorphisms are canonical on $\{s,\id\}$.
\end{lemma}


%IST IM Appendix



\begin{proof} 
	
	
	Let $\psi$ be the following formula:$$\psi(x_1,x_2,y_1,y_2):=\overline{\id}(x_1,y_1)\wedge \overline{\id}(x_1,y_2)\wedge \overline{\id}(x_2,y_1)\wedge \overline{\id}(x_2,y_2).$$
	
	
		Let furthermore be $R_{\id}$ the ternary relation defined by the formula
	$$\sigma(x_1,x_2,x_3):= (s\cup\id)(x_1,x_2) \wedge (s\cup\id)(x_2,x_3)  \wedge s(x_1,x_2). $$
$\sigma$ has the property that $\sigma \wedge s(x_1,x_2)   \wedge  \id(x_2,x_3)$ and $\sigma \wedge \id(x_1,x_2)  \wedge s(x_2,x_3)$
	are satisfiable, but the formula $\sigma\wedge \id(x_1,x_2)   \wedge  \id(x_2,x_3)$ is not satisfiable.
	
	
	
	
	If there exist no $\{s,\id\}$-symmetric polymorphism then item (2) in Lemma \ref{symmetric+formulaslemma} is not satisfied. Therefore, by Lemma \ref{lem: make things unequal} we can assume that there exists a formula $\varphi'$ such that
	
	 \begin{align*}
	 &\varphi'\wedge\psi(x_1,x_2,x_3,x_4) \wedge s(x_1,x_2)   \wedge  \id(y_1,y_2) \\
	 \text{and~}&\varphi' \wedge\psi(x_1,x_2,x_3,x_4)\wedge \id(x_1,x_2)  \wedge s(y_1,y_2)
	 \end{align*}
	 	are satisfiable and the formula $\varphi \wedge s(x_1,x_2)   \wedge  s(y_1,y_2)$ is not satisfiable (we denote this property with $\bigstar$).

	
	
	
	We define 
	 \begin{align*}
	 \varphi_s(x_1,x_2,x_3,x_4) :=& \varphi'(x_1,x_2,x_3,x_4) \wedge\psi(x_1,x_2,x_3,x_4)\\ &\wedge (s\cup \id)(x_1,x_2) \wedge (s\cup \id)(x_3,x_4).
	 \end{align*}
	Now we define the 4-ary relation $R$ as follows:
	
	

	
	
	
	
	
	
	
	
	
	\begin{align*}
	\delta(x_1,x_2,x_3,x_4):= &s(x_1,x_3)\wedge s(x_1,x_4) \wedge s(x_2,x_3) \wedge s(x_2,x_4)\\
	&\wedge \exists y_1,y_2,y_3: (\varphi_s(x_1,x_2,y_1,y_2) \wedge R_{\id}(y_1,y_2,y_3)\\& \wedge \varphi_s(y_2,y_3,x_3,x_4))\\
	&\wedge \exists z_1,z_2:(R_{\id}(x_1,x_2,z_1) \wedge \varphi_s(x_2,z_1,z_2,x_3)\\&\wedge R_{\id}(z_2,x_3,x_4)	)
	\end{align*}
	
	
	
	
	The formulas $\delta \wedge s(x_1,x_2)  \wedge \id(x_3,x_4) $ and $\delta \wedge \id(x_1,x_2)  \wedge s(x_3,x_4)$ are satisfiable.
	To see this note that we have free amalgamation (with respect to the flexible atom) in the structure $\mathfrak{B}$; we can clue  tuples that satisfy $\varphi_s$ with tuples from relation $R_{\id}$ and fill all missing edges with the flexible atom $s$. This is possible since we ensured with $\psi$ that the relevant entries of these tuples are not equal.
	
	A second observation is the following:
	\begin{align*}
	u\in R \Rightarrow  (s(u_1,u_2)  \wedge \id(u_3,u_4))  \vee   (\id(u_1,u_2)  \wedge s(u_3,u_4))
	\end{align*}
	This is because of the second and third line in the defining formula. Assume that for $u\in R$ the formula $s(u_1,u_2)  \wedge s(u_3,u_4)$ holds. Then there exist $y_1,y_2,y_3$ such that $\varphi_s(x_1,x_2 y_1,y_2) \wedge \varphi_s(y_2,y_3,x_3,x_4)$ holds. But this is by $\bigstar$ only possible if $\id(y_1,y_2) \wedge \id(y_2,y_3)$ holds. This is a contradiction since $R_{\id }(y_1,y_2,y_3)$ holds. 
	The same argument works for proving that $\neg ( \id(u_1,u_2)  \wedge \id(u_3,u_4))$ holds.

	
	
	Let  $E_{s,\id}$ be the 4-ary relation defined as
	
		\begin{align*}
	(a_1,\ldots,a_4) \in E_{s,\id} :\Leftrightarrow (s\cup \id)(a_1,a_2)\wedge (s\cup \id)(a_3,a_4) \wedge (s(a_1,a_2) \Leftrightarrow s(a_3,a_4))
	\end{align*}
	We finally use $R$ to get a primitive positive definition of $E_{s,\id}$.
	
	
	
	
	\begin{align*}
	(a_1,\ldots,a_4) \in E_{s,\id} \Leftrightarrow \exists y_1, y_2: (R(a_1,a_2,y_1,y_2) \wedge R(y_1,y_2,a_3,a_4))
	\end{align*}
	 This definition works since for elements in $R$  the free predicate $s$ holds between all its entries whenever  the predicate $\id$  does not hold.  The same free amalgamation argument as before proves the claim.
	

	Since we found a primitive positive definition for the relation $E_{\id,s}$, we know that all polymorphisms of $\mathfrak{B}$ have to preserve this relation. But this is by the definition of $E_{\id,s}$ nothing else than saying that all polymorphisms are $\{\id,s\}$-canonical.\qed\end{proof}







\begin{lemma}\label{lemma: a id canonical implies sym or projections}
	Let $\mathfrak{B}$ be a normal representation of a finite, integral, symmetric $\mathbf{A}\in \rra$ with a flexible atom $s$. Let $a \not\leq \id$ be an atom such that all polymorphisms of $\mathfrak{B}$ are $\{a,\id\}$-canonical. Then either there exists an $\{a,\id\}$-symmetric polymorphism or all polymorphisms are a projection on $\{a,\id\}$.
\end{lemma}

\begin{proof}The  polymorphisms of $\mathfrak{B }$ induce an idempotent operation clone on the set $\{a,\id\}$. Assume this clone does not contain projections only.
	Since we know then that one of the cases in Theorem \ref{post} applies we make a case distinction.

	\underline{Case 1:} Assume there exists a polymorphism $f$ of $\mathfrak{B}$ that induces a majority operation on $\{a,\id\}$. Then consider tuples $x,y,z\in B^3$ such that $$(\id,\id,a)(x,y), ~(\id,a,\id)(y,z), \text{~ and ~} (\id , a,a)(x,z).$$
	If we apply $f$ on these tuples we get on $f(x), f(y)$ and $f(z)$ a substructure that contains a forbidden triple. Therefore, $f$ cannot be a majority operation on $\{a,\id\}$.
	
	\underline{Case 2:} Assume there exists a polymorphism $f$ of $\mathfrak{B}$ that induces a  minority operation on $\{a,\id\}$. Then consider tuples $x,y,z\in B^3$ such that $$(\id,a,a)(x,y), ~(a,a,\id)(y,z), \text{~ and ~} (a , s,a)(x,z).$$
	 Note that such tuples exist since $s$ is a flexible atom.
	If we apply $f$ on these tuples we get on $f(x), f(y)$ and $f(z)$ a substructure that contains a forbidden triple. By the minority operation we get $\id(f(x),f(y))$ and  $\id(f(y),f(z))$, but since $f$ is an edge-conservative polymorphism, we also have $[a\cup s](f(x), f(z))$. This is a contradiction and therefore $f$ can not be a minority operation on $\{a,\id\}$.
	Therefore, item (1) or (2) in Theorem \ref{post} hold. A polymorphism that induces one of these two operations from (1) or (2)  in Theorem \ref{post} on the set  $\{a,\id\}$ is by definition an  $\{a,\id\}$-symmetric polymorphism.
	This proves the lemma. \qed\end{proof}



\begin{lemma}\label{lemma:a id symm means a}
	Let $\mathfrak{B}$ be a normal representation of a finite, integral, symmetric $\mathbf{A}\in \rra$ with a flexible atom $s$. Let $a \not\leq \id$ be an atom and $f$ an $\{a,\id \}$-canonical polymorphism of $\mathfrak{B}$ such that $f$ is $\{a,\id \}$-symmetric. Then $\bar{f}(a,\id)=a=\bar{f}(\id,a)$ holds.
\end{lemma}
\begin{proof}
	The other possibility is $\bar{f}(a,\id)=\id=\bar{f}(\id,a)$, which is not possible since tuples $x,y,z \in B^2$ with $$(a,\id)(x,y), ~ (\id,a)(y,z), \text{~ and ~} (a,a)(x,z)$$ would give a forbidden triple on the induced substructure of $f(x), f(y)$ and $f(z)$.\qed\end{proof}







%\subsection{A Special Independence Lemma}\label{subsection:special independece}
%\textcolor{red}{
%The following lemma is of the same spirit as Lemma \ref{symmetric+formulaslemma}. It gives a connection between the existence  of a special type of polymorphism (in this case an injective one) and primitively positively definable relations. In the terminology of Lemma \ref{symmetric+formulaslemma} an injective, binary polymorphism $f$ is a polymorphism that is $\{a,\id\}$-symmetric with $\bar{f}(\id,a)=a$ for all $a\in A_0$. }
%
%\begin{lemma}\label{lemma:injectiveindependence}
%	Let $\mathfrak{B}$ be a normal representation of a finite, integral, symmetric $\mathbf{A}\in \rra$. Then the following are equivalent:
%	\begin{enumerate}
%		\item $\mathfrak{B}$ has an injective binary polymorphism $g$.
%		\item  For all atoms $a \not \leq \id$ and $b  \not \leq \id$ and every primitive positive formula $\varphi$ such that $\varphi \wedge \id(x_1,x_2)   \wedge  b(y_1,y_2)$  and $\varphi \wedge a(x_1,x_2)  \wedge \id(y_1,y_2)$ are satisfiable over $\mathfrak{B}$, the formula $\varphi \wedge a(x_1,x_2)   \wedge  b(y_1,y_2)$ is also satisfiable over $\mathfrak{B}$.
%		\item For every finite $F\subset B^2$ there exists a homomorphism $h_F$ from the substructure of  $\mathfrak{B}^2$ induced by $F$ to $\mathfrak{B}$ that is injective.
%	\end{enumerate}
%	
%	
%\end{lemma}
%
%
%\begin{proof} The proof is analogous to the proof of Lemma \ref{symmetric+formulaslemma}.
%	
%	
%	The implication from (1) to (2) follows directly by applying the injective polymorphisms on tuples from the relation defined by $\varphi$.\medskip
%	
%	For the implication from (2) to (3) let $F$ be a finite set in $V^2$. Without loss of generality we can assume that $F$ is of the form $\{e_1,\ldots, e_n\}^2$ for a large enough $n\in \mathbb{N}$.
%	To construct $h_F$ consider the formula $\varphi_0$ with variables $x_{i,j}$ for $1\leq i,j \leq n$ that is the conjunction of all atomic formulas $R(x_{i_1,j_1}, x_{i_k,j_k})$ such that $R(e_{i_1}, e_{i_k})$ and $R(e_{j_1}, e_{j_k})$ hold in $\mathfrak{B}$. Note that this formula states exactly which relations hold on $F$ as a substructure of $\mathfrak{C}^2$.
%	
%	Let $P$ be the set of pairs $((i_1,j_1),(i_2,j_2))$ with $(i_1,i_2) \not=(j_1,j_2)$ such that 
%	%	\begin{align*}
%	%	&a\cup \id(e_{i_1}, e_{i_2}) \\
%	%	\textup{and~}& a\cup \id(e_{j_1}, e_{j_2}) \\
%	%	\textup{and~}&( a(e_{i_1}, e_{i_2}) \vee  a(e_{j_1}, e_{j_2}) )\\
%	%	\textup{and~}&( \id(e_{i_1}, e_{i_2}) \vee  \id(e_{j_1}, e_{j_2}) ).
%	%	\end{align*}
%	%	
%	
%	
%	
%	$$\id(e_{i_1}, e_{i_2}) \vee  \id(e_{j_1}, e_{j_2}) $$
%	holds.
%	If we show that the formula 
%	$$\psi:=\varphi_0 \wedge \bigwedge_{((i_1,j_1),(i_2,j_2)) \in P}  \overline{\id}(x_{i_1,j_1},x_{i_2,j_2})$$
%	is satisfiable by an assignment $w$, we get the claimed homomorphisms by setting $h(e_i,e_j):= w(x_{i,j})$. 
%	
%	To prove the satisfiability of $\psi$ we do an inductive argument over the size of subsets $I$ of $P$. 	For the inductive beginning consider an element $((i_1,j_1),(i_2,j_2))\in P$. Without loss of generality we have that $\overline{\id}(i_1,i_2)$ holds. Therefore the assignment $a(x_{i,j}):= e_i$ witness satisfiability of the formula $\varphi_0 \wedge  \overline{\id}(x_{i_1,j_1},x_{i_2,j_2})$. 	For the inductive step let $I\subset P$ be of size $m$ and assume that the statement is true for subsets of size $m-1$. Let  $p_1=((u_1,v_1),(u_2,v_2)) $ and $p_2=((u_1',v_1'),(u_2',v_2')) $ be two elements from $I$. 
%	We define the following formula
%	$$\psi_0:=\varphi_0 \wedge \bigwedge_{((i_1,j_1),(i_2,j_2))\in I\setminus\{p_1,p_2\}}  \overline{\id}(x_{i_1,j_1},x_{i_2,j_2}).$$
%	
%	Then by the inductive assumption the formulas $\psi_0 \wedge \overline{\id}(x_{u_1,v_1},x_{u_2,v_2})$ and 
%	$\psi_0 \wedge \overline{\id}(x_{u_1',v_1'},x_{u_2',v_2'})$ are satisfiable. The assumptions on elements in $P$ give us that also $\psi_0 \wedge \overline{\id}(x_{u_1,v_1},x_{u_2,v_2}) \wedge \id(x_{u_1',v_1'},x_{u_2',v_2'})$ 
%	and $\psi_0 \wedge \id(x_{u_1,v_1},x_{u_2,v_2}) \wedge \overline{\id}(x_{u_1',v_1'},x_{u_2',v_2'})$ are satisfiable; since $a\cup \id$ is a primitively positively definable relation for every atom $a$ we are done otherwise. 
%		Now we can apply the assumption of (2) and get that also $\psi_0 \wedge \overline{\id}(x_{u_1,v_1},x_{u_2,v_2}) \wedge \overline{\id}(x_{u_1',v_1'},x_{u_2',v_2'})$ is satisfiable which proves the inductive step. 
%	\medskip
%	
%	The direction from (3) to (1) is a standard application of K\"onig's tree lemma. For a reference look for example in TODO
%\qed\end{proof}


%\begin{lemma}
%		Let $\mathfrak{B}$ be a normal representation with a flexible atom $s$ and an atom $a\not\leq \id$ such that $a\not= s$. Then the 4-ary  relation that satisfies defined by $\neg( \id(x_1,x_2) \wedge \id(x_3,x_4))$ is primitively positively definable.
%\end{lemma}
%
%\begin{proof}
%Consider the primitive positive formula 
%$$\varphi(x_1,\ldots x_4):\Leftrightarrow \exists y_1,y_2,   a(x_2,y_1)\wedge s(x_1,y_2) \wedge a(y_2,x_3) \wedge s(y_1,x_4)$$
%\qed\end{proof}

\begin{lemma}\label{lemma:not(2) implies no symm}
	Let $\mathfrak{B}$ be a normal representation of a  finite, integral, symmetric  $\mathbf{A}\in \rra$ with a flexible atom $s$. If $\mathfrak{B}$ does not have a binary injective polymorphism then $\mathfrak{B}$ does not have a $\{s,\id\}$-symmetric polymorphism.
\end{lemma}
\begin{proof}
	Assume for contradiction that $\mathfrak{B }$ has an $\{s,\id\}$-symmetric polymorphism $f$.
	By Lemma \ref{lemma:a id symm means a} the only possibility is that $\bar{f}(s,\id)=s=\bar{f}(\id,s)$ holds.
	Let $a\in A_0$ be an arbitrary atom and let $x,y\in B^2$ such that $\id(x_1,y_1)$ and $a(x_2,y_2)$ hold. We can choose $z\in B^2$ such that $(\id, s)(z,x)$ and $(\id, a)(z,y)$ hold. By the assumption on $f$ we get $s(f(z),f(x))$. This implies also that $a(f(x),f(y))$ holds, since otherwise we would induce a forbidden substructure. Since we chose $a$ and $x$ and $y$ arbitrary and by an analogous argument for the change of the coordinates we get that $f$ is $\{a,\id\}$-symmetric with $\bar{f}(a,\id)=a=\bar{f}(\id,a)$ for all $a\in A_0$. This means that $f$ is injective, which contradicts the assumption.\qed\end{proof}





%\begin{lemma}\label{lemma:not(2) implies no symm}
%	Let $\mathfrak{B}$ be a normal representation of a  finite, integral, symmetric  $\mathbf{A}\in \rra$ with a flexible atom $s$. If (2) in Lemma \ref{lemma:injectiveindependence} does not hold for atoms $a\leq \id$ and $b\leq \id$ then there is no $\{s,\id\}$-canonical polymorphism $f$ with $f(s,\id)=s=f(\id,s)$.
%\end{lemma}
%
%
%\begin{proof}
%	
%	
%	\underline{Claim 1:} There is no $\{a,\id\}$-canonical polymorphism $f$  with $\bar{f}(a,\id)=a=\bar{f}(\id,a)$.
%	
%	Let $\varphi$ be the formula that witness that (2)  in Lemma does not hold for atoms $a$ and $b$. This formula defines a 4-ary relation $R$ such that there exists a tuple $x\in R$ with $\id(x_1,x_2)$ and $a(x_3,x_4)$ as well as a tuple $y\in R$ with $b(y_1,y_2)$ and $\id(y_3,y_4)$. By the assumption on $\varphi$ there exist no tuple $z$ in $R$ such that $b(c_1,c_2)$ and $a(c_3,c_4)$.
%	Assume that an $\{a,\id\}$-canonical polymorphism $f$ with $\bar{f}(a,\id)=a=\bar{f}(\id,a)$ exists, then $f$ is also a $\{b,\id\}$-canonical polymorphism with $\bar{f}(b,\id)=\id=\bar{f}(\id,b)$ since $f$ preservers the relation $R$. Note that this woks since we can find for all $x_1,x_2, y_1,y_2 \in B$ with $\id(x_1,x_2)$  and $b(y_1,y_2)$  elements $x_3,x_4,y_3,y_4$ such that $x,y\in R$. This is a contradiction to Lemma \ref{lemma:a id symm means a} and proves the claim.
%
%Assume there exists an $\{s,\id\}$-canonical polymorphism $f$ with $\bar{f}(s,\id)=s=\bar{f}(\id,s)$.
%Let $x,y\in B^2$ such that $\id(x_1,y_1)$ and $a(x_2,y_2)$. We can choose $z\in B^2$ such that $(\id, s)(z,x)$ and $(\id, a)(z,y)$. By the assumption on $f$ we get $s(f(z),f(x))$. Note that this implies that $a(f(x),f(y))$ holds, since otherwise we would induce a forbidden substructure. Since we chose $x$ and $y$ arbitrary and by an analogous argument for the change of the coordinates we get that $f$ is $\{a,\id\}$-canonical with $\bar{f}(a,\id)=a=\bar{f}(\id,a)$. This contradicts Claim 1 and  proves therefore the statement.\qed\end{proof}


%\begin{lemma}
%		Let $\mathfrak{B}$ be a normal representation with a flexible atom $s$. If (2) in Lemma does not hold for atoms $a$ and $b$ then all polymorphism are $\{a,\id\}$-canonical and $\{b,\id\}$-canonical.
%\end{lemma}
%
%
%
%\begin{proof}
%Let $\varphi$ be the formula that witness that (2)  in Lemma does not hold for atoms $a$ and $b$. This formula defines a 4-ary relation $R$ such that there exists a tuple $x\in R$ with $\id(x_1,x_2)$ and $a(x_3,x_4)$ as well as a tuple $y\in R$ with $b(y_1,y_2)$ and $\id(y_3,y_4)$. 
%By the assumption on $\varphi$ there exist no tuple $z$ in $R$ such that $b(c_1,c_2)$ and $a(c_3,c_4)$.
% We will use also a relation $R'$ that is permutation of the coordinates of the tuples of $R$ like follows
% $$x\in R' :\Leftrightarrow R(x_3,x_4,x_1,x_2)$$
%
%Now we define a new 4-ary relation $Q$ by
%
%\begin{align*}
%x\in Q:\Leftrightarrow \exists y_1,y_2,z_1,z_2,u_1,u_2. & R'(x_1,x_2,y_1,y_2) \wedge R(y_1,y_2,z_1,z_2) \wedge R'(z_1,z_2, u_1,u_2 )\\
%&\wedge R(u_1,u_2,x_3,x_4) \wedge (a\cup \id)(x_1,x_2) \wedge(a\cup \id)(x_3,x_4)
%\end{align*}
%Since $\mathfrak{B}$ has a flexible atom, this relation witness that all polymorphisms are $\{a,\id\}$-canonical.
%
% 
%\qed\end{proof}

%\begin{lemma}
%		Let $\mathfrak{B}$ be a normal representation with a flexible atom $s$. If for every atom $a \not\leq \id$ there exist an  $\{a,\id \}$-canonical polymorphism such that $f(a,\id)=a=f(\id,a)$ holds, then there exists an injective binary polymorphism of $\mathfrak{B}$.
%\end{lemma}
%\begin{proof}
%	Assume that no binary injection exists. Then (2) in Lemma does not hold and therefore by Lemma all polymorphisms are $\{a,\id\}$-canonical and $\{b,\id\}$-canonical. 
%	Let $f_a$ and $f_b$ be the polymorphisms that exist by assumption. Then the polymorphism $$g(x,y):= f_a( f_b(x,y), f_b(y,x) )$$ shows that (2) in Lemma holds. This is a contradiction.
%\qed\end{proof}








Now we are able to prove the main result of this section.





\begin{proof}[of Proposition \ref{binaryinjectionNPhard}]
Since $\mathfrak{B }$ is finitely bounded $\csp(\mathfrak{B} )$ is in NP.
	Assume that $\mathfrak{B }$ has  no injective binary polymorphism.
%	By Lemma \ref{lemma:injectiveindependence} there exist atoms $a  \not \leq \id$ and $b  \not \leq \id$ such that (2) in Lemma \ref{lemma:injectiveindependence} does not hold.
	Then Lemma \ref{lemma:not(2) implies no symm}  implies that there exists no $\{s,\id\}$-symmetric polymorphism
	%with $\bar{f}(s,\id)=s=\bar{f}(\id,s)$. By Lemma \ref{lemma:a id symm means a} this means there exists no $\{s,\id\}$-symmetric polymorphism 
	and therefore by Lemma \ref{lemma: no a id symm implies a id canonical} all polymorphisms are $\{s,\id\}$-canonical. Lemma \ref{lemma: a id canonical implies sym or projections} implies then that all polymorphisms are Boolean projections on $\{s,\id\}$. 
	It is easy to see that therefore $\HSPf(\{\Pol(\mathfrak{B }) \}  )$ contains a 2-element algebra where all operations are projections. This proves by Theorem \ref{theo:hardness} the NP-hardness of $\csp(\mathfrak{B })$.\qed\end{proof}







%
%\section{Proof of NP-Hardness}\label{section:hardness}
%
%%
%%\begin{theorem}
%%	If the orbit structure of a normal representation has a trivial subalgebra then there exist a uniformly continuous minor preserving map $\Pol( \mathfrak{B} ) \rightarrow \Proj$. In this case $\csp(\mathfrak{B})$ is NP-complete.
%%\end{theorem}
%
%
%The goal of this section is to prove our main result.
%In order to do this three things are left. Recall that in  Section \ref{section:finite type structure} we ended with the existence of a trivial subalgebra of $\Pol(\mathfrak{O})$. This implies among other things that there exist atoms $a,b\in A_0$ such that there exists no \emph{canonical} $\{a,b\}$-symmetric polymorphism.  Since the Independence Lemma \ref{symmetric+formulaslemma} is about $\{a,b\}$-symmetric polymorphisms (without canonical) we would like to show that they can also not exist.
%This will be done with the help of an injective polymorphism in the first part of this section. 
%
%In our proof strategy we then reached the point that we apply the Independence Lemma: The absence of an $\{a,b\}$-symmetric polymorphism implies the existence of relations for which a certain implication does not hold. In the third part of the section we use these relations to prove that all the polymorphisms are $\{a,b\}$-canonical and therefore $\Pol(\mathfrak{B })$ induces operation clone on a Boolean domain. 
%
%The second part ensures that this clone is the projection clone. 
%Since the first and the second part are conceptually equal we ordered the parts that way.
%
%%If this clone would not be the projection clone then there exists a Schaefer operation. We already know that such a n operation can not be 
%For the whole section assume that $\mathfrak{B }$ is a normal representation of a finite, integral, symmetric $\mathbf{A}\in \rra$ with a flexible atom.

==> IndependenceLemma5.tex <==
\section{The Independence Lemma}\label{section:independence}


This section introduces a key method of our analysis. The ``independence lemma'' transfers the absence of a special partially canonical polymorphism into the existence of certain relations of arity $4$ that are primitively positively definable in $\mathfrak{B}$.
These relations will later help us to prove the NP-hardness of $\csp(\mathfrak{B})$.
A lemma of a similar type  appeared for example as Lemma 42 in\cite{RandomMinOps}.


\begin{definition}\label{orbits}Let $\mathfrak{B }$ be a relational structure. A set $O\subset B^n$ is called an \emph{$n$-orbit} of $\Aut(\mathfrak{B })$ if $O$ is preserved by all $\alpha \in \Aut(\mathfrak{B })$ and for all $x,y \in O$ there exists $\alpha \in \Aut(\mathfrak{B })$ such that $\alpha(x)=y$.

	\end{definition}


\begin{lemma}\label{symmetric+formulaslemma}
	Let $\mathfrak{B}$ be a homogeneous structure with finite relational signature. Let $a$ and $b$ be 2-orbits of $\Aut(\mathfrak{B })$ such that $a$, $b$, and $(a\cup b)$ are primitively positively definable in $\mathfrak{B }$. 
	Then the following are equivalent:
	\begin{enumerate}
		\item $\mathfrak{B}$ has an $\{a,b\}$-canonical polymorphism $g$ that is $\{a,b\}$-symmetric with $\overline{g}(a,b)=\overline{g}(b,a)=a$.
		\item  For every primitive positive formula $\varphi$ such that $\varphi \wedge a(x_1,x_2)   \wedge  b(y_1,y_2)$ and $\varphi \wedge b(x_1,x_2)  \wedge a(y_1,y_2)$ are satisfiable  over $\mathfrak{B}$, the formula $\varphi \wedge a(x_1,x_2)   \wedge  a(y_1,y_2)$ is also satisfiable  over $\mathfrak{B}$.
		\item For every finite $F\subset B^2$ there exists a homomorphism $h_F$ from the substructure of  $\mathfrak{B}^2$ induced by $F$ to $\mathfrak{B}$ that is $\{a,b\}$-canonical with  $\overline{h_F}(a,b)=\overline{h_F}(b,a)=a$.
	\end{enumerate}
	
	
\end{lemma}


%ist im appendix

\begin{proof}
	The implication from (1) to (2) follows directly by applying the symmetric polymorphisms on tuples from the relation defined by $\varphi$.\medskip
	
	For the implication from (2) to (3) let $F$ be a finite set in $B^2$. Without loss of generality we may assume that $F$ is of the form $\{e_1,\ldots, e_n\}$ for a large enough $n\in \mathbb{N}$.
	To construct $h_F$ consider the formula $\varphi_0$ with variables $x_{i,j}$ for $1\leq i,j \leq n$ that is the conjunction of all atomic formulas $R(x_{i_1,j_1},\ldots, x_{i_k,j_k})$ such that $R(e_{i_1}, \ldots, e_{i_k})$ and $R(e_{j_1}, \ldots, e_{j_k})$ hold in $\mathfrak{B}$. Note that this formula states exactly which relations hold on $F$ as a substructure of $\mathfrak{B}^2$.
	Let $P$ be the set of pairs $((i_1,i_2),(j_1,j_2))$ such that 
	\begin{align*}
	&(a\cup b )(e_{i_1}, e_{i_2}) \\
	\textup{and~}& (a\cup b (e_{j_1}, e_{j_2}) \\
	\textup{and~}&( a(e_{i_1}, e_{i_2}) \vee  a(e_{j_1}, e_{j_2}) ).\\
	\textup{and~}&( b(e_{i_1}, e_{i_2}) \vee  b(e_{j_1}, e_{j_2}) ).
	\end{align*}
		If we show that the formula 
	$$\psi:=\varphi_0 \wedge \bigwedge_{((i_1,i_2),(j_1,j_2)) \in P}  a(x_{i_1,j_1},x_{i_2,j_2})$$
	is satisfiable by an assignment $s$, we get the claimed homomorphisms by setting $h(e_i,e_j):= s(x_{i,j})$. 
	We prove the satisfiability of $\psi$  by induction over the size of subsets $I$ of $P$. 
	For the inductive beginning consider an element $((i_1,i_2),(j_1,j_2)) \in P$. Without loss of generality we have that $a(i_1,i_2)$ holds. Therefore the assignment $s(x_{i,j}):= e_i$ witnesses satisfiability of the formula $\varphi_0 \wedge  a(x_{i_1,j_1},x_{i_2,j_2})$. 
	For the inductive step let $I\subset P$ be of size $m$ and assume that the statement is true for subsets of size $m-1$. Let  $p_1=((u_1,u_2),(v_1,v_2)) $ and $p_2=((u_1',u_2'),(v_1',v_2')) $ be two elements from $I$. 
	We define the following formula
	$$\psi_0:=\varphi_0 \wedge \bigwedge_{((i_1,i_2),(j_1,j_2)) \in I\setminus\{p_1,p_2\}}  a(x_{i_1,j_1},x_{i_2,j_2}).$$
	Then by the inductive assumption the formulas $\psi_0 \wedge a(x_{u_1,v_1},x_{u_2,v_2})$ and 
	$\psi_0 \wedge a(x_{u_1',v_1'},x_{u_2',v_2'})$ are satisfiable. The assumptions on the elements in $P$ give us that also $\psi_0 \wedge a(x_{u_1,v_1},x_{u_2,v_2}) \wedge b(x_{u_1',v_1'},x_{u_2',v_2'})$ 
	and $\psi_0 \wedge b(x_{u_1,v_1},x_{u_2,v_2}) \wedge a(x_{u_1',v_1'},x_{u_2',v_2'})$ are satisfiable; since $a\cup b$ is a primitive positive definable relation we are done otherwise.  But then we can apply the assumption of (2) and get that also $\psi_0 \wedge a(x_{u_1,v_1},x_{u_2,v_2}) \wedge a(x_{u_1',v_1'},x_{u_2',v_2'})$ is satisfiable, which proves the inductive step. 
	
	
	The direction from (3) to (1) is a standard application of K\"onig's tree lemma. For a reference see for example Lemma 42 in\cite{RandomMinOps}. \qed\end{proof}



%
%
%
%\begin{lemma}\label{lem:definability}
%	Let $\mathfrak{B}$ be a normal representation of a finite, integral, symmetric relation algebra $\mathbf{A}$ with a flexible atom $s$. Let $a$ and $b$ be atoms such that there exists no $\{a,b\}$-symmetric polymorphism. Then all polymorphisms are canonical on $\{a,b\}$.
%\end{lemma}
%
%
%
%
%
%\begin{proof}
%		Let $\varphi_a$ and $\varphi_b$ be the two formulas that exist by Lemma \ref{symmetric+formulaslemma} to witness that there exist no symmetric polymorphism $g$ with $\overline{g}(a,b)=a$ or $\overline{g}(a,b)=b$. 
%	We define the following formulas
%	\begin{align*}
%	&\varphi'_a:= \varphi_a \wedge [a\cup b](x_1,x_2)  \wedge [a \cup b](y_1,y_2),\\
%	&\varphi'_b:= \varphi_b \wedge [a\cup b](x_1,x_2)  \wedge [a \cup b](y_1,y_2).
%	\end{align*}
%	
%	Without loss of generality, we can assume that they define two 4-ary relations $R_a$, and $R_b$ such that
%	
%	\begin{align}
%	&u \in R_a \Rightarrow \neg ( a(u_1,u_2)  \wedge a(u_3,u_4)) \text{~and}\\
%	&u \in R_b \Rightarrow \neg ( b(u_1,u_2)  \wedge b(u_3,u_4)).
%	\end{align}
%	
%	
%	
%	\underline{Step 1:} The Relation $Q_{ab}$ with
%	
%	
%	\begin{align*}
%	Q_{a,b}(x_1,x_2,x_3,x_4):= \exists y_1,y_2: R_a(x_1,x_2,y_1,y_2)\wedge R_b( y_1,y_2,x_3,x_4)
%	\end{align*}
%	
%	
%	satisfies the following condition
%	$$u\in Q_{a,b} \Rightarrow \neg( a(u_1,u_2) \wedge b(u_3,u_4)) \wedge \overline{\id}(u_1,u_4)$$
%	
%	
%	
%	
%	\underline{Step 1:} There exist relations $R_a'$ and $R_b'$ that satisfy (1) and (2)	and also
%		\begin{align}
%	&u \in R_a' \Rightarrow \overline{\id}(u_1,u_3)  \wedge \overline{\id}(u_1,u_4))  \wedge \overline{\id}(u_2,u_3)  \wedge \overline{\id}(u_2,u_4) \text{~and}\\
%	&u \in R_b' \Rightarrow  \overline{\id}(u_1,u_3)  \wedge \overline{\id}(u_1,u_4))  \wedge \overline{\id}(u_2,u_3)  \wedge \overline{\id}(u_2,u_4) .
%	\end{align}
%	
%	In order to prove this, we show the claim for $R_a'$.
%	
%	
%	\begin{align*}
%	R_a'(x_1,x_2,x_3,x_4):= 
%	&\wedge \exists y_1,y_2,y_3,y_4,t_1,t_2,t_3,t_4: R_a(t_1,t_2,x_1,x_2) \wedge R_a(x_3,x_4,t_3,t_4)\\
%	&\wedge R_a(y_1,y_2,t_1,t_2)\wedge R_a(t_3,t_4,y_3,y_4)  \wedge R_b(y_1,y_2,y_3,y_4)\\
%	&\wedge \exists z_1,z_2,z_3,z_4,s_1,s_2,s_3,s_4: R_b(s_1,s_2,x_1,x_2) \wedge R_b(x_3,x_4,s_3,s_4)\\
%	&\wedge R_b(z_1,z_2,s_1,s_2)\wedge R_b(s_3,s_4,z_3,z_4)  \wedge R_a(z_1,z_2,z_3,z_4)
%	\end{align*}
%	
%	
%	
%	
%\qed\end{proof}



